These Magic Moments: Differentiable Uncertainty Quantification of Radiance Field Models

This paper introduces a novel approach to uncertainty quantification for radiance fields by leveraging higher-order moments of the rendering equation. Uncertainty quantification is crucial for downstream tasks including view planning and scene understanding, where safety and robustness are paramount. However, the high dimensionality and complexity of radiance fields pose significant challenges for uncertainty quantification, limiting the use of these uncertainty quantification methods in high-speed decision-making. We demonstrate that the probabilistic nature of the rendering process enables efficient and differentiable computation of higher-order moments for radiance field outputs, including color, depth, and semantic predictions. Our method outperforms existing radiance field uncertainty estimation techniques while offering a more direct, computationally efficient, and differentiable formulation without the need for post-processing. Beyond uncertainty quantification, we also illustrate the utility of our approach in downstream applications such as next-best-view (NBV) selection and active ray sampling for neural radiance field training. Extensive experiments on synthetic and real-world scenes confirm the efficacy of our approach, which achieves state-of-the-art performance while maintaining simplicity.

==> sec/5_Limitations.tex <==
\section{Limitations} \label{sec:limitations}
The proposed method computes pixel-wise higher-order moments of rendered features by considering the probabilistic optical model underlying radiance fields.
These higher-order moments are computed using the differentiable framework of existing radiance field models, namely NeRF and 3DGS models.

While the proposed approach is a means of estimating aleatoric uncertainty, uncertainty arising from the data used to train the model and uncertainty in the model itself, it is unable to estimate epistemic uncertainty, uncertainty due to a lack of data.
This estimation of epistemic uncertainty remains a challenge for radiance field models and so far solutions have only been proposed by leveraging voxels to represent unseen regions of a scene.

Furthermore, the proposed variance computations were not used as an additional training signal for radiance field models.
Interestingly, leveraging the standard evidential regression cost functions \cite{amini2020deep} does not lead to better performance, nor does it degrade the results.
We aim to study this phenomenon in future work and determine whether higher-order moments are useful as an additional training signal for radiance field models.
